Spatially Varying Nanophotonic Neural Networks

The explosive growth of computation and energy cost of artificial intelligence has spurred strong interests in new computing modalities as potential alternatives to conventional electronic processors. Photonic processors that execute operations using photons instead of electrons, have promised to enable optical neural networks with ultra-low latency and power consumption. However, existing optical neural networks, limited by the underlying network designs, have achieved image recognition accuracy far below that of state-of-the-art electronic neural networks. In this work, we close this gap by embedding massively parallelized optical computation into flat camera optics that perform neural network computation during the capture, before recording an image on the sensor. Specifically, we harness large kernels and propose a large-kernel spatially-varying convolutional neural network learned via low-dimensional reparameterization techniques. We experimentally instantiate the network with a flat meta-optical system that encompasses an array of nanophotonic structures designed to induce angle-dependent responses. Combined with an extremely lightweight electronic backend with approximately 2K parameters we demonstrate a reconfigurable nanophotonic neural network reaches 72.76\% blind test classification accuracy on CIFAR-10 dataset, and, as such, the first time, an optical neural network outperforms the first modern digital neural network -- AlexNet (72.64\%) with 57M parameters, bringing optical neural network into modern deep learning era.

==> sections/figures/exp_cls.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main/fig3.png}
    \caption{\textbf{Validation of \shortname~as a versatile computational camera}. (a) Feature maps of \shortname~on ImageNet dataset. (b) Recognition performance of the ImageNet-designed \shortname~instance, on ImageNet and other downstream datasets (CIFAR-100, Flowers102 and Pet37) using the universal optical encoder, and the transfer-learned electronic decoder. These findings validate that the proposed camera, with a fixed optical encoder, can generalize to diverse tasks by adapting the electronic backend.} 
    \label{fig:exp-imagenet}
\end{figure*}


==> sections/figures/measure.tex <==
\begin{figure*}[t]    
    \centering
    \begin{tabular}{c}
        \includegraphics[width=.9\textwidth]{./figures/suppl/measures/measures_1.png} \\ \hdashline       
        \includegraphics[width=.9\textwidth]{./figures/suppl/measures/measures_2.png}   	               
    \end{tabular}
    \caption{Experimentally measured image feature samples produced by \shortname~ (images formed by traditional hyperbolic lens in four corners are discarded.)}
    \label{fig:measure-samples}
\end{figure*}

==> sections/figures/overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main/fig1.pdf}
    \caption{\textbf{Spatially varying nanophotonic neural networks}. (a) Illustration of the proposed opto-electronic network, which comprises a nanophotonic array front-end that optically encodes the scene into multichannel image features, and a lightweight electronic back-end that performs the final prediction, in a programmable manner, for image classification or semantic segmentation; (b) Each metalens is designed for specific large and angularly varying point spread functions that comprise the feature kernels of the early network layers which vary over the sensor. These kernels are learned electronically using a spatially varying reparameterization. (c) We learn large kernels by factorizing them into a cascade of smaller ones. (d) The representative spatially varying kernels over space (first row) and the corresponding kernel standard deviation at each spatial location. }    
    \label{fig:metaonn-overview}
\end{figure*}


==> sections/figures/phase_profiles.tex <==
\begin{figure*}[t]    
    \centering
    \begin{tabular}{c}
        \includegraphics[width=\textwidth]{./figures/suppl/phase/SV.png}   	\\ \hdashline
        \includegraphics[width=\textwidth]{./figures/suppl/phase/ImageNet.png}   	               
    \end{tabular}
    \caption{Inverse designed phase profiles of \shortname~(Top: CIFAR-10 design; Bottom: ImageNet design)}
    \label{fig:phase_profiles}
\end{figure*}

==> sections/figures/res_seg.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{example-image}    
    \end{subfigure}
      \hfill
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{example-image}
    \end{subfigure}
    %\caption{\textbf{Semantic segmentation with \shortname}}   
    \caption{\textbf{\shortname~as a versatile computational camera for large-scale ImageNet classification and PASCAL-VOC semantic segmentation.}}   
    \label{fig:res-imagenet-seg}
\end{figure*}


==> sections/figures/sim_cls.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main/fig2.png}
    \caption{\textbf{Experimental validation of \shortname~}. (a) Close-up of the metalens array camera and a metalens array device before mounting; (b) Experimental setup, consisting of an OLED display placed at the designed object distance, and a large-area CMOS sensor is placed at the focal plane of the metalens array. Both are synchronized for data capture; (c) Spatially-varying PSF visualization on a $3\times 3$ sampling grid of incident angles. We show here four representative kernels; (d) Side-by-side comparisons of the experimental measurements and the corresponding ground truth feature channels. ``Real-valued'' denotes the target feature channel, that is the negative image feature subtracted from positive image features post-convolution.}
    \label{fig:exp-val-cifar10-1}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main/fig2-1.png}
    \caption{\textbf{Experimental measurements of a fabricated chip of a design for CIFAR-10 image classification}. (a) Qualitative assessment of the experimental measurements compared with the ground truth feature channels. ``Real-valued'' again denotes here the target feature channels via subtraction of the negative from the  positive image features post-convolution. (b) The confusion matrices of the experimental and simulation results on CIFAR-10 testing dataset. }
    \label{fig:exp-val-cifar10-2}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main/cls_vis_res.pdf}
    \caption{\textbf{Experimental (top-2) classification (probability) results on random samples from CIFAR-10 test set}. \textcolor{ForestGreen}{Green} and \textcolor{Orange}{Orange} colored labels under the images denote the correct and incorrect predictions, respectively.}
    \label{fig:cls-vis-res}
\end{figure*}


==> sections/tables/ablation.tex <==
\begin{table}
    \renewcommand{\arraystretch}{2}
    \centering
    \caption{\textbf{Ablation and Complexity Experiments for the Proposed Design Variant (LKSV)}: We report the number of multiply–accumulate (MAC) operations, the inference runtime (TIME) and the number of parameters (\# of PARAMS) for the optical and electronic parts of different models. The runtime is reported for a NVIDIA GTX 1080Ti GPU; note that the true optical runtime is only a function of the optical path length and is $\approx3$ ps in our implementation. We report here the runtime numbers of the optical model component when implemented electronically for reference, \ie, higher is better. The labels SK/LK refer to small and large kernel respectively; SI/SV indicate spatially invariant and spatially varying respectively. * denotes large kernel and/or spatially varying convolutional layer learned \textit{without} low-dimensional reparameterization. 
    ACC denotes the blind testing accuracy on the CIFAR-10 dataset. The result of AlexNet is also listed as a reference.}
    \label{table:ablation}
    \vspace{10pt}
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\textsc{Model}} & \multirow{2}{*}{\textsc{ACC}} & \multicolumn{2}{c|}{\textsc{MAC}} & \multicolumn{2}{c|}{\textsc{TIME}} & \multicolumn{2}{c|}{\textsc{\# of PARAMS}}  \\ \cline{3-8}
    & & \textsc{Optical} $\uparrow$ & \textsc{Electronic} $\downarrow$ & \textsc{Optical} $\uparrow$ & \textsc{Electronic} $\downarrow$  & \textsc{Optical} $\uparrow$ & \textsc{Electronic} $\downarrow$ \\ \hline
    \multirow{2}{*}{AlexNet}  &  \multirow{2}{*}{72.64 \%} & - & 174.85 M  & -  & 70.58 us & - & 57.03 M \\ 
    &  & - &  100 \% & - & 100 \% & - & 100 \% \\ \hline
    \multirow{2}{*}{SKSI}  &  \multirow{2}{*}{65.45 \%} & 243.20 K & 125.30 K  & 0.41 us  & 2.64 us & 0.25 K & 2.03 K \\ 
    &  & 66.00 \% &  34.00 \% & 13.56 \% & 86.44 \% & 10.94 \% & 89.06 \% \\ \hline

    \multirow{2}{*}{LKSI*} & \multirow{2}{*}{67.13 \%} & 5.78 M & 125.30 K & 3.54 us  & 2.64 us  & 5.65 K  & 2.03 K  \\         
    & & 97.88 \% & 2.12 \% & 57.25 \% &  42.75 \% & 73.52 \% & 26.48 \% \\ \hline
    

    \multirow{2}{*}{LKSI} & \multirow{2}{*}{71.64 \%} & 5.78  M & 125.30 K & 3.54 us  & 2.64 us  & 5.65 K  & 2.03 K  \\         
    & & 97.88 \% & 2.12 \% & 57.25 \% &  42.75 \% & 73.52 \% & 26.48 \% \\ \hline
    
    \multirow{2}{*}{SKSV*} & \multirow{2}{*}{57.69 \%} & 1.41 M & 125.30 K  & 27.72 us  & 2.64 us  & 6.52 K & 2.03 K \\        
    & & 91.83 \% & 8.17 \%  & 91.30 \% &  8.70 \% & 76.21 \% & 23.79 \% \\ \hline


    \multirow{2}{*}{SKSV} & \multirow{2}{*}{71.14 \%} & 1.41 M & 125.30 K  & 27.72 us  & 2.64 us  & 6.52 K & 2.03 K \\        
    & & 91.83 \% & 8.17 \%  & 91.30 \% &  8.70 \% & 76.21 \% & 23.79 \% \\ \hline

    \multirow{2}{*}{LKSV} & \multirow{2}{*}{\textbf{73.80} \%} & 34.59 M  & 125.30 K  & 302.66 us  & 2.64 us & 38.92 K & 2.03 K \\   
    & &  \textbf{99.64} \%  & \textbf{0.36} \%  & \textbf{99.14} \% &  \textbf{0.86} \%  &   \textbf{95.03} \%  &   \textbf{4.97} \%  \\ \hline        

    \end{tabular}
\end{table}
